Duality and small functors

The homotopy theory of small functors is a useful tool for studying various questions in homotopy theory. In this paper, we develop the homotopy theory of small functors from spectra to spectra, and study its interplay with Spanier-Whitehead duality and enriched representability in the dual category of spectra. We note that the Spanier-Whitehead duality functor $D\colon \mathrm{Sp}\rightarrow \mathrm{Sp}^{\mathrm{op}}$ factors through the category of small functors from spectra to spectra and construct a new model structure on the category of small functors, which is Quillen equivalent to $\mathrm{Sp}^{\mathrm{op}}$. In this new framework for the Spanier-Whitehead duality, $\mathrm{Sp}$ and $\mathrm{Sp}^{\mathrm{op}}$ are full subcategories of the category of small functors and dualization becomes just a fibrant replacement in our new model structure.

==> symbols.tex <==

%
% Classes in model categories
%

\newcommand{\inj}{\text{-inj}}
\newcommand{\proj}{\ensuremath{\text{-proj}}}
\newcommand{\cell}{\text{-cell}}


\newcommand{\sS}{\ensuremath{\cal S}}
\newcommand{\Sp}{\ensuremath{\textup{Sp}}}

\newcommand{\funS}{^\sS}
\newcommand{\funSop}{^{\sS^{\op}}}
\newcommand{\Set}{\ensuremath{\textup{\bf Set}}}
\newcommand{\gpscat}{\ensuremath{\textup{Gps}}}
\newcommand{\topcat}{\ensuremath{\textup{Top}}}
\newcommand{\Gps}{\ensuremath{\textup{Gps}}}

\newcommand{\op}{{\ensuremath{\textup{op}}}}
\newcommand{\opp}{^\op}
\newcommand{\fin}{{\ensuremath{\textup{fin}}}}

\DeclareMathOperator{\Hor}{\ensuremath{\textup{Hor}}}
\DeclareMathOperator{\Ho}{\ensuremath{\textup{Ho}}}
\newcommand{\Rmod}{\ensuremath{R-\textup{mod}}}
\newcommand{\modR}{\ensuremath{{\textup mod}-R}}

%
% Diagram
%

\newcommand{\dgrm}[1]{\ensuremath{\smash{\underset{\widetilde{\hphantom{#1}}}{#1}} \mathstrut}}


%
% Arrows and constructions
%


\newcommand{\surj}{\ensuremath{\twoheadrightarrow}}%     % Surjektion 
%\newcommand{\inj}{\ensuremath{\hookrightarrow}}%         % Injektion
                            % \rightarrowtail früher   ------   Georg's notation

\newcommand {\cofib} {\ensuremath{\hookrightarrow}}

\newcommand {\fibr} {\ensuremath{\twoheadrightarrow}}

\newcommand {\trivcofib} {\ensuremath{\xhookrightarrow \sim}}

\newcommand {\trivfibr} {\ensuremath{\tilde\twoheadrightarrow}}

\newcommand {\we} {\ensuremath{\xrightarrow \sim}}

\newcommand{\orbit}[1]{\ensuremath{\overset {#1} {\underset \ast \downarrow}}}

\newcommand{\vertmap}[2]{\ensuremath{\overset {#1} {\underset #2 \downarrow}}}

\newcommand{\two}[2]{\ensuremath{\genfrac{}{}{0pt}{0}{#1}{#2}}}


\newcommand{\mhyphen}{\ensuremath{\mathrel{\mathstrut}}}



%\newcommand{\domain}[1]{\ensuremath{\gothic d({#1})}}
%\newcommand{\range}[1]{\ensuremath{\gothic r({#1})}}
%\newcommand{\domain}[1]{\ensuremath{\mathrm{dom}({#1})}}
%\newcommand{\range}[1]{\ensuremath{\mathrm{codom}({#1})}}


\DeclareMathOperator{\domain}{\textup{dom}}
\DeclareMathOperator{\codom}{\textup{codom}}

\DeclareMathOperator{\cof}{\textup{cof}}
\DeclareMathOperator{\fib}{\textup{fib}}

\DeclareMathOperator{\hocolim}{\textup{hocolim}}
\DeclareMathOperator{\holim}{\textup{holim}}


%\DeclareMathOperator{\inj}{\textup{inj}}
%\DeclareMathOperator{\proj}{\textup{proj}}
%\DeclareMathOperator{\cell}{\textup{cell}}

\DeclareMathOperator{\pres}{\textup{\bf Pres}}
\DeclareMathOperator{\MC}{\textup{MC}}

\newcommand{\cal}[1]{\ensuremath{\mathcal #1}}

%
% Theorem numeration and style.
%

\newtheorem {theorem1}{Theorem}[section]
\newtheorem {theorem}[theorem1]{Theorem}
\newtheorem*{theorem_nonum}{Theorem}
\newtheorem {corollary}[theorem1]{Corollary}
\newtheorem {proposition}[theorem1]{Proposition}
\newtheorem {lemma}[theorem1]{Lemma}
\theoremstyle{definition}
\newtheorem {definition}[theorem1]{Definition}
\newtheorem*{definition_nonum}{Definition}
\newtheorem {cond}[theorem1]{}
\newtheorem {example}[theorem1]{Example}
\theoremstyle{remark}
\newtheorem {remark}[theorem1]{Remark}
\newtheorem {recall}[theorem1]{Reminder}


%
% Calligraphic letters
%

\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}

%
% Categories Names
%

\newcommand{\cat}[1]{\ensuremath{\EuScript #1}}

\newcommand{\Pow}[1]{\ensuremath{\textup{Pow}\, #1}}

\newcommand{\Top}{\ensuremath{\calT\textup{op}}}
\newcommand{\Cat}{\ensuremath{\cal C\textup{at}}}
\newcommand{\Ord}{\ensuremath{\cal O\textup{rd}}}
\newcommand{\Topstar}{\ensuremath{\calT\textup{op}_*}}
\newcommand{\Ab}{\ensuremath{\cal{A}\textup{b}}}
\newcommand{\Sets}{\ensuremath{\cal{S}}\emph{ets} }
\newcommand{\Cmplx}[1]{\ensuremath{\partial#1\textsl{mod}}}
\newcommand{\Lmod}[1]{\ensuremath{#1\textsl{-mod}}}
%
% General mathematical symbols
%

\DeclareMathOperator{\Map}{\ensuremath{\textup{Map}}}
\DeclareMathOperator{\Hom}{\ensuremath{\textup{Hom}}}
\DeclareMathOperator{\map}{\textup{map}}
\DeclareMathOperator{\successor}{\textup{succ}}

\newcommand{\NN}{\ensuremath{\mathbb{N}}}
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\QQ}{\ensuremath{\mathbb{Q}}}

\newcommand{\func}[3]{\ensuremath{#1\colon #2\rightarrow #3}}

%\DeclareMathOperator{\colim}{\textup{colim}}
%\DeclareMathOperator{\holim}{\textup{holim}}
%\newcommand{\holim}{\ensuremath{\mathop{\textup{holim}}}}

\newcommand{\colim}{\ensuremath{\mathop{\textup{colim}}}}
\newcommand{\Sing}{\ensuremath{\mathop{\textup{Sing}}}}


\newcommand{\invlim}{\ensuremath{\varprojlim}}
\newcommand{\rarrowonto}{\ensuremath{\rightarrow}}
\newcommand{\coker}{\ensuremath{\textup{coker}}}
\def\hopushout{\ensuremath{\textsl{hopush}}}
\def\hopush{\ensuremath{\textsl{hopush}}}
\def\id{\ensuremath{\textsl{id}}}
\def\Lan{\ensuremath{\textup{Lan}}}
\newcommand{\hopull}{\ensuremath{\textsl{hopull}}}
\def\push{ \ensuremath{\textsl{pushout}} }
\def\pull{ \ensuremath{\textsl{pullback}} }
\def\opp{\ensuremath{\textit{opp}}}
\newcommand{\Lcplx}[1]{\ensuremath{\partial#1mod}}
\newcommand{\Rcplx}[1]{\ensuremath{\partial#1^{\opp}mod}}
\newcommand{\LRcplx}[2]{\ensuremath{\partial#1#2^{\opp}mod}}

%
% Shortcuts
%
\newcommand{\GothC}{\ensuremath{\cal{C}}}
\newcommand{\larrow}{\leftarrow}
\newcommand{\rarrow}{\rightarrow}
\newcommand{\Id}{\ensuremath{\textup{Id}}}
\newcommand{\IG}{\ensuremath{\textup{I}G}}

\newcommand{\obj}[1]{\ensuremath{\textup{obj}(#1)}}
\newcommand{\mor}[1]{\ensuremath{\textup{mor}(#1)}}
\newcommand{\overcat}{\ensuremath{\!\downarrow\!}}
\newcommand{\im}[1]{\ensuremath{\textsl{im}(#1)}}
\newcommand{\mytimes}{\ensuremath{\bar{\times}}}
\def\ev{\ensuremath{\textit{ev}}}
\newcommand{\tev}[1]{\ensuremath{\tilde{\textit{ev}}_{#1}}}

\newcommand{\etale}{\'etale }

\newcommand{\Adamek}{Ad\'amek }
\newcommand{\Rosicky}{Rosick\'y }
\newcommand{\Kunneth}{K\"unneth }
\newcommand{\Poincare}{Poincar\'e }
\newcommand{\Vopenka}{Vop\v enka }
\newcommand{\Vopenkas}{Vop\v enka's }
\newcommand{\Mardesic}{Marde{\v{s}}i{\'c} }


%%% some commands from Georg
%%% Georg's commands %%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\geo}[1]{\marginpar{ \raggedleft\sffamily{\scriptsize Georg: #1}}}%
\newcommand{\bor}[1]{\marginpar{ \raggedleft\sffamily{\scriptsize Boris: #1}}}%


\newcommand{\toh}[1]{\ensuremath{\stackrel{#1}{\rightarrow}}}%    
                                                     % Pfeil mit Hochstellung

\newcommand{\co}{\colon\thinspace}%                      % Doppelpunkt ohne Abstand
\newcommand{\mc}[1]{\ensuremath{\cat{#1}}}%          % \euscript  
\newcommand{\sm}[2]{\ensuremath{#1\smash[b]{\wedge\,}#2}}% Smash
%%% Wedge heißt \vee oder \bigvee                        %%%%%%%%%%%%%%%%%

\newcommand{\aus}{\raisebox{1pt}{\ensuremath{\,{\scriptstyle\in}\,}}}%
                                                         % Element von
\newcommand{\eps}{\varepsilon}%                          % epsilon
%%%\newcommand{\colim}{\operatorname*{colim}}%              % colim
%%%\newcommand{\coker}{\operatorname{coker\,}}%             % Cokern
\newcommand{\sk}{\operatorname{sk}}%                     % Skelett
\newcommand{\cosk}{\operatorname{cosk}}%                 % Koskelett
%%%\newcommand{\im}{\operatorname{im}}%                     % Bild
%%%\newcommand{\holim}{\operatorname*{holim\,}}%            % holim 
%%%\newcommand{\hocolim}{\operatorname*{hocolim\,}}%        % hocolim 
\newcommand{\Rlim}{\operatorname*{lim^1}}%               % abgeleiteter Limes 
\newcommand{\frei}{\,\_\!\_\,}%                          % Freizeichen
\newcommand{\hofi}{\ensuremath{\mathfrak{Hofi}\,}}%      % Hofi-Funktor
\newcommand{\cone}{\ensuremath{\mathfrak{Cone}\,}}%      % Cone-Funktor
%%%\newcommand{\id}{\operatorname{id}}%                     % Identität
\newcommand{\8}{\ensuremath{\infty}}                     % Unendlich
\newcommand{\Tot}{\operatorname{Tot}}%                   % Tot  
\newcommand{\RKan}{\operatorname*{RKan}}%                % RKan 
\newcommand{\LKan}{\operatorname*{LKan}}%                % LKan
\newcommand{\HoRKan}{\operatorname*{HoRKan\,}}%          % HoRKan 
\newcommand{\HoLKan}{\operatorname*{HoLKan\,}}%          % HoLKan
\newcommand{\cosim}{\ensuremath{\underline{\Delta}^*}}%  % cosimplizial 
%\newcommand{\surj}{\ensuremath{\twoheadrightarrow}}%     % Surjektion 
%\newcommand{\inj}{\ensuremath{\hookrightarrow}}%         % Injektion
                            % \rightarrowtail früher

\newcommand{\ho}[1]{\ensuremath{H\!o({#1})}}%      % Homotopiekategorie 
%%%%% \newcommand{\ho}[1]{\ensuremath{H\!o\hrl{#1}\hrr}}%% Homotopiekategorie 

\newcommand{\bth}{\raisebox{1pt}{\ensuremath{\,\scriptstyle \geq\,}}}%
                                                         % ein ordentliches >=
\newcommand{\sth}{\raisebox{1pt}{\ensuremath{\,\scriptstyle \leq\,}}}%
                                                         % ein ordentliches <=
\newcommand{\uber}{\raisebox{1pt}{\ensuremath{\,{\scriptstyle > }\,}}}%
\newcommand{\unter}{\raisebox{1pt}{\ensuremath{\,{\scriptstyle < }\,}}}%
\newcommand{\ent}{\raisebox{1pt}{\ensuremath{\,{\scriptstyle \subseteq }\,}}}%
\newcommand{\umf}{\raisebox{1pt}{\ensuremath{\,{\scriptstyle \supseteq }\,}}}%
%\newcommand{\copost}{\ensuremath{{\rm coPost}}}%         % coPost-Kategorie
\newcommand{\x}{\operatorname*{\times}}%                 % 

%%%%%%%% Für Pushout- und Pullbackdiagramme rechte Winkelzeichen
\newcommand{\pullback}{\displaystyle \cdot\!\!\lrcorner}%
%%%\newcommand{\hopushout}{h-\displaystyle \cdot\!\!\lrcorner}%
\newcommand{\winkel}{\ulcorner\hspace{-3pt}\raisebox{1pt}{\ensuremath{\cdot}}}%
\newcommand{\pushout}{\raisebox{-3pt}{\ensuremath{\displaystyle \winkel}}}%

%%%%%%%% Verzierungen  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ul}[1]{\underline{#1}}%                     % Unterstreichen
\newcommand{\ol}[1]{\overline{#1}}%                     % Überstreichen
\newcommand{\wt}[1]{\widetilde{#1}}%                     % Schlange
\newcommand{\wh}[1]{\widehat{#1}}%                       % Hut

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% Einige Hom-Mengen            %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\stabhom}[2]{\ensuremath{\hel#1,#2\her}}%
%%%\newcommand{\Hom}[3]{\ensuremath{{\rm Hom}_{#1}\hrl#2,#3\hrr}}%
\newcommand{\Aut}{\ensuremath{\rm Aut}}%
\newcommand{\gradhom}[4]{\ensuremath{{\rm Hom}_{#1}^{#2}\hrl#3,#4\hrr}}%
\newcommand{\Ext}[4]{\ensuremath{{\rm Ext}_{#1}^{#2}\hrl#3,#4\hrr}}%

%%%\newcommand{\map}{\ensuremath{{\rm map}}}%  % für Modellkategorien
\renewcommand{\hom}{\ensuremath{{\rm hom}}}%% redefined

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% Diagramme etc.               %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\diag}[2]{ \begin{align} \begin{split} \xymatrix{#1} \end{split} \label{#2} \end{align}}%    
%%%%%%%% numeriertes zentriertes Diagramm mit Label %%%%%%%%%%%%%%%
%%%%%%%% centertags-Packet                          %%%%%%%%%%%%%%%

\newcommand{\diagr}[1]{ \begin{equation*} \xymatrix{#1} \end{equation*}}%
%%%%%%%%                         Diagramm           %%%%%%%%%%%%%%%

\def\setrefstep#1{\setcounter{enumi}{#1}}
            % Dieser Befehl setzt den Z"ahler in der enumerate-Umgebung neu. 
            % Damit kann man eine neue Umgebung aufmachen, die schon bei einer
            % gewissen Zahl anfängt zu zählen. Dies geht mit folgendem
            % Befehl:
            % \begin{enumerate}\setrefstep{1}\item Teil 2\end{enumerate}
            % Fängt erst bei 2 an zu zählen.

%%%\newcommand{\Ref}[1]{\hrl\ref{#1}\hrr}        % klammert Verweise ein

\newcounter{zahl}%
\newenvironment{punkt}{\begin{list}{{\rm{(\roman{zahl})}}}%
    {\usecounter{zahl}%
     \setlength{\leftmargin}{0pt} \setlength{\itemindent}{4pt} \setlength{\topsep}{2pt} \setlength{\parsep}{2pt} }}%
    {\end{list}}%
%%%%%%%% Listenumgebung, siehe auch Latex-Begleiter Seite 60 %%%%%%


